HyFusion: Enhanced Reception Field Transformer for Hyperspectral Image Fusion

Hyperspectral image (HSI) fusion addresses the challenge of reconstructing High-Resolution HSIs (HR-HSIs) from High-Resolution Multispectral images (HR-MSIs) and Low-Resolution HSIs (LR-HSIs), a critical task given the high costs and hardware limitations associated with acquiring high-quality HSIs. While existing methods leverage spatial and spectral relationships, they often suffer from limited receptive fields and insufficient feature utilization, leading to suboptimal performance. Furthermore, the scarcity of high-quality HSI data highlights the importance of efficient data utilization to maximize reconstruction quality. To address these issues, we propose HyFusion, a novel Dual-Coupled Network (DCN) framework designed to enhance cross-domain feature extraction and enable effective feature map reusing. The framework first processes HR-MSI and LR-HSI inputs through specialized subnetworks that mutually enhance each other during feature extraction, preserving complementary spatial and spectral details. At its core, HyFusion utilizes an Enhanced Reception Field Block (ERFB), which combines shifting-window attention and dense connections to expand the receptive field, effectively capturing long-range dependencies while minimizing information loss. Extensive experiments demonstrate that HyFusion achieves state-of-the-art performance in HR-MSI/LR-HSI fusion, significantly improving reconstruction quality while maintaining a compact model size and computational efficiency. By integrating enhanced receptive fields and feature map reusing into a coupled network architecture, HyFusion provides a practical and effective solution for HSI fusion in resource-constrained scenarios, setting a new benchmark in hyperspectral imaging. Our code will be publicly available.

==> sections/1.5_related.tex <==
\section{Related Works}


%In recent years, image fusion has also been applied to the task of HSI and MSI fusion. Unlike ordinary MSI images with three or more channels, HSI typically have a much larger number of channels. Therefore, there are certain differences between traditional image fusion and HSI fusion. This chapter will introduce traditional HSI fusion methods and image fusion methods based on deep learning architectures.

%\subsection{Optimization and Decomposition based approach}
%In \cite{16}, an innovative MSI pan-sharpening framework was introduced, aiming to fuse LR-MSI and an HR-panchromatic image (a single-band image with high spatial resolution) of the same scene to produce an image with enhanced spectral and spatial resolutions. Additionally, leveraging the sparse or low-rank priors of HSIs, several image fusion frameworks based on sparse representation or low-rank models have been developed for HSI super-resolution or HR-MSI/LR-HSI fusion \cite{7,8,17,18,19}. For instance, \cite{7} proposed an SR method for LR-HSI, framing HR-HSI prediction as a joint learning task of the HSI dictionary and sparse codes, exploiting the spatial-spectral sparsity of HSIs. Moreover, \cite{8} introduced a group spectral embedding-based HR-MSI/LR-HSI fusion method, which investigates the manifold structures of spectral bands and the low-rank properties of HR-HSIs. Similarly, a spatial and spectral fusion model was proposed in \cite{17}, employing sparse matrix factorization to fuse remote sensing images with HR-MSI and LR-HSI. Another image fusion framework was presented in \cite{18}, relying on spectral unmixing and sparse coding to merge HR-MSI and LR-HSI. Additionally, \cite{19} introduced a coupled sparse tensor factorization framework for HR-MSI and LR-HSI fusion, formulating the dictionary and core tensor estimation as a coupled tensor factorization problem. Since these traditional methods depend on specific image priors, such as sparsity or low-rank assumptions, their performance may degrade in real-world scenarios that deviate from these assumptions. Moreover, optimization-based approaches typically require high-precision computation, making it challenging to deploy these algorithms on standard AI chips due to difficulties in parallelization (e.g., eigendecomposition is commonly used in these methods). Consequently, reducing computational complexity while maintaining strong performance is highly sought after.

%\subsection{Deep learning-based approach}
%Deep learning (DL) methods have made significant contributions to the field of image processing and HSI fusion. With advancements in the field, DL has become the mainstream approach for HSI fusion due to its greater efficiency and superior performance compared to optimization-based methods.

%\subsubsection{CNN-based approach}
%With the advancements in DL technology, including the powerful representation learning capabilities of CNNs, several SR frameworks for LR-HSI or the fusion of HR-MSI and LR-HSI have been proposed in recent years. For example, a 3D-CNN approach \cite{20} was employed to fuse LR-HSI and HR-MSI to reconstruct an HR-HSI, where dimensionality reduction was applied to the HSI before feature fusion to significantly lower computational complexity. Additionally, \cite{21} formulated and addressed a blind HR-MSI and LR-HSI fusion problem using DL, where the estimation of the observation model and the fusion process were iteratively and alternately optimized during the SR reconstruction. Moreover, \cite{22} introduced an HSI reconstruction algorithm with a data-driven prior inspired by optimization principles, where the prior was learned based on both the local coherence and dynamic properties of HSIs. Moreover, MSSJFL was proposed \cite{23} to jointly learn multi-scale spatial-spectral features for HR-MSI and LR-HSI fusion. In addition, PZRes-Net \cite{24}, a lightweight progressive zero-centric residual network, was presented for HSI super-resolution, where the spectral-spatial separable convolution operations with dense connections were used to efficiently learn the residual image. Dual-UNet \cite{25} architecture with a multi-stage details injection strategy was presented for fusing HR-MSI and LR-HSI, where a multi-scale spatial-spectral attention was utilized. Furthermore, DHIF-Net \cite{26} was proposed, it leveraged an end-to-end optimization strategy of iterative spatial-spectral regularization was implemented. On the other hand, an unregistered and unsupervised mutual Dirichlet-Net was presented \cite{27} for LR-HSI super-resolution.% An Interpretable deep neural network designed for HR-MSI/LR-HSI fusion was proposed in \cite{28}. An interpretable deep model named by spatial–spectral dual-optimization model-driven deep network was also presented in \cite{29} for HR-MSI/LR-HSI fusion. 
%\subsubsection{Generative Adversarial Network based approach}
%In recent years, Generative Adversarial Networks (GANs) have become a popular topic in the field of image processing. GANs have shown great capabilities in generating high-quality images, restoring damaged images, transforming image styles, and enhancing image quality. In terms of image generation, DCGAN \cite{DCGAN} and StyleGAN \cite{stylegan} are commonly used methods that can generate realistic images. For image restoration, pix2pix \cite{p2p} is a commonly used approach. In image transformation, CycleGAN \cite{CycleGAN2017} and style transfer are common methods that can convert images with different styles into images with similar styles. In terms of image enhancement, SRGAN \cite{100} and GAN-based image enhancement are widely used methods that can improve image quality and resolution. 

%Ma et al. proposed Pan-GAN \cite{MA2020110}, which is an unsupervised generative adversarial network fusion method based on the pan-sharpening framework. In this approach, the authors used a generator that undergoes adversarial learning with a spectral discriminator and a spatial discriminator. Xiao et al. \cite{111} proposed a physics-based GAN network for fusing HSI and MSI. The network consists of a generator network and three discriminator networks. The fused image is then fed into a simple and effective recursive module, where the spatial and spectral details of the image can be refined through multiple iterations, enhancing useful learning features.
%\subsubsection{Autoencoder based approach}
%Autoencoder is commonly used in image processing for image compression. By reducing the dimensionality of the image, it achieves image compression by decreasing the image size. Autoencoder consists of an encoder and a decoder, which are separately trained. The encoder maps the input to a lower-dimensional space, and the decoder reconstructs the original image from the encoded representation. Autoencoder can also be used for image denoising. Denoising Autoencoder \cite{DAE} is a neural network used to remove noise from images. It takes a noisy image as input and reconstructs it into a clean, noise-free image, allowing the model to learn denoising capabilities. Autoencoder can also be used for image feature extraction. In tasks such as image classification and object detection, the network extracts useful features from the images by learning a compact representation.

%In the task of HSI fusion, Autoencoder is also a commonly used method. The main idea of this approach is to use a autoencoder to learn the mapping relationship between the LR-HSI and the LR-MSI, thus achieving the fusion of HR-MSI and LR-HSI. Arian et al. \cite{cae} proposed CAE, which is a multispectral fusion method based on autoencoder. In this method, a trained CAE network generates the original pan-sharpened image from the spatially degraded image. Then, the LR-MSI image is inputted into the trained CAE to generate the estimated HR-MSI. 

